Mining Frequent Patterns in Evolving Graphs

Given a labeled graph, the frequent-subgraph mining (FSM) problem asks to find all the $k$-vertex subgraphs that appear with frequency greater than a given threshold. FSM has numerous applications ranging from biology to network science, as it provides a compact summary of the characteristics of the graph. However, the task is challenging, even more so for evolving graphs due to the streaming nature of the input and the exponential time complexity of the problem. In this paper, we initiate the study of the approximate FSM problem in both incremental and fully-dynamic streaming settings, where arbitrary edges can be added or removed from the graph. For each streaming setting, we propose algorithms that can extract a high-quality approximation of the frequent $k$-vertex subgraphs for a given threshold, at any given time instance, with high probability. In contrast to the existing state-of-the-art solutions that require iterating over the entire set of subgraphs for any update, our algorithms operate by maintaining a uniform sample of $k$-vertex subgraphs with optimized neighborhood-exploration procedures local to the updates. We provide theoretical analysis of the proposed algorithms and empirically demonstrate that the proposed algorithms generate high-quality results compared to baselines.

==> sections/discussion.tex <==
% !TEX root = ../main.tex
\section{Previous Discussion and Ideas}
\label{sec:prel}

%\section{Frequent subgraph mining}
%Given a directed labeled static graph $G=(V,E, \nodelabel, \edgelabel)$ with node labels $\nodelabel: V\to \nodelabelspace$ and edge labels  $\edgelabel: E\to \edgelabelspace$.
%A stream of updates to the graph $\Upd = \{(t,\edit)\}$ where $t$ is a timestamp and $\edit\in \{(\type, \entity, \info)\}$ contains information about update.
%$\entity$ is either a node or an edge to be altered, $\type$ is $+$, if the entity is added and $-$, if it is removed; $\info$ carries necessary labeling information.
%Several updates can have the same timestamp.
%
%Graph $\sgr=(\sgrnodes,\sgredges)$ is a subgraph of $G$, if $\sgrnodes\subseteq V$,  $\sgredges\subseteq E$, $\sgrnodelabel(u) =\nodelabel(u)$ and $\sgredgelabel((u,v)) =\edgelabel((u,v))$ for any node $u$ and edge $(u,v)$ in $\sgr$.
%Subgraph isomorphism is defined as usually: function $f$, which maps nodes of a subgraph to nodes of the graph, such that all labels are matched.
%More formally: an injective function of nodes $f:\sgrnodes \to V$, such that $\sgrnodelabel(u) = \nodelabel(f(u))$ for all $v\in \sgrnodes$; $(f(u), f(v))\in E$ for all $(u,v)\in \sgredges$ and $\sgredgelabel((u,v)) = \sgredgelabel((f(u),f(v)))$.
%
%Following standards from recent papers, frequency of subgraph $\sgr$ is defined based of minimum image support (MNI).
%Let $F(\sgr)=\{f_1,\dots,f_m\}$ be a set of isomorphisms of $\sgr$ on $G$.
%Let $F(u)=\{f_1(u),\dots,f_m(u)\}$ be a set of all possible images of $u$ in $F(\sgr)$.
%Define support as $s(\sgr)=\min\{|F(u)|\quad \forall u\in \sgrnodes\}$.
%
%Subgraph $\sgr$ is called frequent if its support is above threshold $\threshold$.	
%
%Denote state of graph $G$ by time $t$ as $G_t = (V_t, E_t,\nodelabel, \edgelabel)$.
%The task is to retrieve frequent subgraphs (for a fixed threshold \threshold or top-$k$ frequent subgraphs) in $G_t$ for every current time $t$.
%
%\section*{General approach}
%Here we consider only edge removal and addition, as all other changes can be done based on these two operations.
%We also consider only connected (induced?) subgraphs.
%
%In dynamic scenario we cannot build structures for compact storage of patterns based on their frequencies, like FP-trees, thus we apply subgraph enumeration trees.
%
%A basic approach described here is based on reverse search method \cite{avis1996reverse} for connected subgraph enumeration.
%An instance of this general method was applied in gSpan \cite{yan2002gspan}.
%Similar to gSpan, we use minimum DFS encoding for subgraphs and construct a prefix tree $\maintree$ of all found patterns.
%Every node of the tree corresponds to an edge, encoded by 5-tuple with 2 numbers for its place in DFS search and 3 items for its labeling.
%Every path from the root is a subgraph, encoded by its minimum DFS code.
%Following \cite{avis1996reverse, yan2002gspan}, there is a bijection between a node of that tree and all possible subgraphs.
%The tree has exponential size, we can truncate it by size of the graph (number of edges $k$).
%
%Every node also contains a set of images of this edge within the subgraph pattern, encoded by the path (If this is large, we can store only sketches).
%Frequency of a subgraph can be calculated as minimum image cardinality of the nodes on the path.
%
%Every addition or removal of an edge $e$ lead to changes in frequencies of subgraphs, which contain $e$.
%Consider only changes in subgraphs with at most $k$ edges (has the same flavor as idea from \cite{ray2014frequent}).
%Using any type of reversed search, we construct a tree $\localtree$ of modified subgraphs with their min-DFS codes and update corresponding paths in the main tree $\maintree$.
%
%If we have a frequency threshold $f$, denote the size of the largest frequent subgraph in $\maintree$ as $k_f$.
%We can set the size of the largest graph in $\localtree$ to be $k_f+1$, ensuring that every possibly-frequent supergraph is kept track of.


%\section{Possible Algorithm}
%Let $H_k$ be the graph of subgraphs of size $k$ build from the original graph $G$, such that there is an edge between two nodes in $H$ if they differ only by one element (edge or vertex, according to how the subgraphs are induced).
%
%Perform a random walk on $H$ to sample subgraphs.
%
%For each sampled subgraph $p \in H$, instantiate a \emph{minimum image subgraph counter} $M_p$.
%The counter has a bit vector $M_p^v$ of size $n$ for each vertex $v \in p$.
%When a subgraph is sampled, the bits corresponding to image of each node in the pattern are set to $1$.
%The frequency of a subgraph is then
%\[
%\min_{v \in p} \sum M_p^v .
%\]
%
%In practice, the but vector can be substituted by a set-size estimator (distinct counter) such as HyperLogLog.
%Also, instead of keeping a counter for each pattern, we can keep only the most frequent ones, by using the SpaceSaving algorithm.
%
%\spara{Questions:}
%\begin{squishlist}
%\item Can we ensure that the sampling is unbiased w.r.t. this definition of frequency?
%\item What happens with automorphic patterns? Do we count them multiplicity times?
%\item How do we grow the pattern size from $k$ to $k+1$ and reuse some of the sampling done?
%\end{squishlist}


\subsection{Streaming setting}
Assume a slightly different problem in the streaming setting.
The input is a dynamic graph in a form of an edge stream, possibly with addition and deletions.
We want to find the frequent subgraphs of size $k$ and an estimate of their frequency for the graph at each timestamp.

\spara{Possible Algorithm.}
The algorithm works by keeping a uniformly random sample of the subgraphs in the graph, which provide a good estimate of the frequency of the (frequent) subgraphs.
The estimates are computed in 2 steps.
\begin{enumerate}
\item A random walk sampler generates a stream of subgraphs of size $k$, one for each step $t$ of the random walk. Each subgraph has an associated probability of being sampled.
\item A reservoir sample \reservoir of this stream contains a uniform sample of size $m$ of the subgraphs in the graph.
\end{enumerate}

Note that the random walker actually generates a stream of visited nodes, and we keep a sliding window of size $k$ to compute the current sample, which is the induced subgraph by the $k$ latest vertices in the random walk.
Each subgraph (or embedding) is thus a set of vertices, with the corresponding induced vertices, and an associated sampling probability.

The random walk sampler collects estimates for the frequency of every subgraph it encounters.
These estimates are used to compute the result for a snapshot of the input graph.
Clearly, the stream of subgraphs generated by the random walk is biased, both by the degree of the vertices included and the shape of the motif underlying the pattern itself.
However, both probabilities can be computed and accounted for.

When an update arrives (edge modification), we check if it affects any of the subgraphs in the reservoir \reservoir.
Three possible cases may happen:
\begin{enumerate}
\item The edge does not intersect any of the subgraphs in \reservoir. In this case, we leave our estimates and result unchanged.
\item Only one of the endpoints of the edge is included in a subgraph in \reservoir. In this case, the induced subgraph does not change. However, its probability of being sampled is now different, because the degree of one of its vertices has changed. So, we can modify the count of the corresponding pattern by $p_{new} / p_{old} \times m/t$. (need to figure out the appropriate formula to take into account the sampling probability of the reservoir).
\item Both endpoints of the edge are included in a subgraph in \reservoir. In this case, the induced subgraph changes. We need to update the counts of both the old pattern and the newly formed one.
The old count should decrease by $p_{old} \times m/t$.
The new count should increase by $p_{new} \times m/t$.
\end{enumerate}

\spara{Implementation note.}
The reservoir \reservoir can be implemented by a hashmap which has vertices as keys, and subgraphs as values. Each subgraph is recoverable from every one of its vertices.

TODO:
\begin{itemize}
\item Figure out correct probabilities for the updates.
\item Prove unbiasedness of the (combined) estimator.
\item Examine special case for k=3 (triangles and wedges), which might be easier to analyze.
\item Determine $m$, the size of \reservoir.
\item Possibly, if the number of patterns to keep estimates of is large, use SpaceSaving to keep only top-k counts.
\end{itemize}


